QPEs as Lense-Thirring precession of super-Eddington flows

Quasi-periodic eruptions (QPEs) are a recently identified class of X-ray transient associated with tidal disruption events by supermassive black holes, and for which there are multiple possible explanations. In this paper we present a simple model which requires the black hole be spinning, be misaligned with the accretion flow (both conditions of which are almost certainly met) and that the accretion rate is a few times the Eddington limit. We speculate that the resulting Lense-Thirring torques force the disc and entrained outflows to precess, leading to increased X-ray flux when the wind-cone is oriented at lower inclinations to the observer. We test the range of parameters for which this model could explain the period and brightness of the QPE events discovered thus far, and make qualitative comparisons between the observed X-ray spectra and lightcurves to those extracted from GR-RMHD simulations. Overall, we find some areas of promising concordance, and identify challenges related to the details of current simulations.

==> QPE_details.tex <==
Source name:GSN069
Peak T: 103 pm 2 eV %from Miniutti+23, quiescence subtracted; note that QPE L and Tpeak decreased through the years
Trough T: 48 pm 2 %Miniutti+19
L peak: 3.4e42 %Lbol QPE, from Miniutti+23; quiescence subtracted
L trough: %will ask Giovanni asap
Mass: 5.99 pm 0.5
Period: 9h %when they were regular ,e.g. see Miniutti+23
% extracted XMM4 0831790701 2019-01-16 134
%https://arxiv.org/pdf/2207.07511.pdf
\\
\medskip


Source name: RXJ1301
Peak T: 125 pm 2 eV % quiescence spectrum subtracted
Trough T: 55 pm 2 eV
L peak: 1e42 %0.3-2keV, couldnt find bol yet
L trough: 1e41 %0.3-2 keV, couldnt find bol yet
Mass: 6.5 pm 0.42
Period: ?? %doesn't really have one, you can use the average of 13 and 20ks from Giustini+20 for now
%flares in 2000 and 2019, 2019 is longer obs with three flares
%https://www.aanda.org/articles/aa/full_html/2020/04/aa37610-20/F1.html
\\
\medskip

Source name: ero-qpe1
Peak T:  262 pm 6 eV %Arcodia+21
Trough T: 130 pm 30 eV % A21; note that this is a rough estimate likely contaminated by background. Quiescence is not securely detected.
L peak: 3.8e43 pm 0.1e43 % A21
L trough: 1.2e41 pm 0.7e41 %same as above, probably an upper limit at `1.6e41 erg s-1
Mass: 5.78 pm 0.55
Period: 19h % quite a large dispersion 3h
% https://www.researchgate.net/publication/351138141_X-ray_quasi-periodic_eruptions_from_two_previously_quiescent_galaxies observation from 27 of July

\\
\medskip

Source name: ero-qpe2
Peak T: 214 pm 30 %quiescence subtracted
Trough T: 76 pm 5 eV
L peak: 4.2e42 pm 0.3e42 %quiesc subtracted
L trough: 5.6e41 pm 0.3e41 cgs %bol
Mass: 4.96 pm 0.54
Period: 2.4h % with 5min dispersion; avg period decreased slightly over 2 years, this is the A21 value
%observation from August
\\
\medskip

Source name: 2MASXJ0249
XMMSL1 J024916.6-041244
Peak T: 165 pm 21
Trough T: 77 pm 7
L peak: 3.4e41 %0.5-2keV
L trough: 1.6e41 % 0.5-2keV
Mass: 5.29 pm 0.55
Period: 9ks %candidate, 1.5 flares only

\\
\medskip

